AC/DC: In-Database Learning Thunderstruck

We report on the design and implementation of the AC/DC gradient descent solver for a class of optimization problems over normalized databases. AC/DC decomposes an optimization problem into a set of aggregates over the join of the database relations. It then uses the answers to these aggregates to iteratively improve the solution to the problem until it converges. The challenges faced by AC/DC are the large database size, the mixture of continuous and categorical features, and the large number of aggregates to compute. AC/DC addresses these challenges by employing a sparse data representation, factorized computation, problem reparameterization under functional dependencies, and a data structure that supports shared computation of aggregates. To train polynomial regression models and factorization machines of up to 154K features over the natural join of all relations from a real-world dataset of up to 86M tuples, AC/DC needs up to 30 minutes on one core of a commodity machine. This is up to three orders of magnitude faster than its competitors R, MadLib, libFM, and TensorFlow whenever they finish and thus do not exceed memory limitation, 24-hour timeout, or internal design limitations.

==> algorithms.tex <==
\section{Algorithms}
\label{SEC:ALGO}

We apply batch gradient-descent (BGD) to optimize the loss function $J(\vec\theta)$ 
over the dataset defined by the query result of a query $Q$ and database $D$. In a BGD
algorithm, two computations are repeated a given number of runs or until convergence of the parameters $\vec\theta$: (1) {\em Point
evaluation}: Given $\vec\theta$, compute the scalar $J(\vec\theta)$;
and (2) {\em Gradient computation}: Given $\vec\theta$, compute
the vector $\grad J(\vec\theta)$. The basic structure of the algorithm is
shown in Algorithm~\ref{algo:bgd}.

\begin{algorithm}[th]
   \caption{BGD with Armijo line search.}
   \label{algo:bgd}
   $\vec\theta \gets $ a random point\;
   \While{not converged yet}{
      $\alpha \gets $ next starting step size \tcp*[f]{Barzilai-Borwein}\;
      $\mv d \gets \grad J(\vec\theta)$\;
      \While{$\left(J(\vec\theta-\alpha \mv d) \geq J(\vec\theta)-\frac
      \alpha 2 \norm{\mv d}_2^2\right)$}{
         $\alpha \gets \alpha/2$ \tcp*[f]{line search}\;
      }
      $\vec\theta \gets \vec\theta - \alpha \mv d$\;
   }
\end{algorithm}

We refer the reader to the excellent review
article~\cite{DBLP:journals/corr/GoldsteinSB14} for more details on fast
implementations of gradient-descent. In particular, our implementation used
the ``adaptive'' Barzilai-Borwein step size adjustment~\cite{MR967848}
recommended in~\cite{MR2144378}.

\subsection{Precomputations}

To illustrate the main idea, we first consider the simplest case when there are no 
categorical features: we rewrite~\eqref{eqn:square:loss} to factor out 
the data-dependent part of these two computations.
A proof of the theorem is in \cite{NNOS2017}~Appendix B. 

\bthm
Let $J(\vec\theta)$ be the function defined in~\eqref{eqn:square:loss}.
Define the matrix $\vec\Sigma = (\sigma_{ij})_{i,j\in [m]}$, 
the vector $\mv c = (c_i)_{i \in [m]}$, and the scalar $s_Y$ by
\begin{eqnarray}
   \vec\Sigma &=& \frac{1}{|Q(D)|} \sum_{(\mv x,y)\in Q(D)} h(\mv x) h(\mv
   x)^\top \label{eqn:sigma}\\
   \mv c &=& \frac{1}{|Q(D)|} \sum_{(\mv x,y)\in Q(D)} y\cdot h(\mv x)\label{eqn:c}\\
   s_Y &=& \frac{1}{2|Q(D)|}\sum_{(\mv x,y)\in Q(D)} y^2.
\end{eqnarray}
Then,
\begin{align}
   J(\vec\theta) &= \frac 1 2 g(\vec\theta)^\top \vec\Sigma g(\vec\theta)
   - \inner{g(\vec\theta), \mv c} + s_Y
   +\frac \lambda 2 \norm{\vec\theta}^2\label{eqn:point:eval}\\
   \grad J(\vec\theta) &= \pd{g(\vec\theta)^\top}{\vec\theta}\vec\Sigma
   g(\vec\theta)-\pd{g(\vec\theta)^\top}{\vec\theta} \mv c+\lambda\vec\theta\label{eqn:gradient}
\end{align}
\label{thm:Sigma:h}
\ethm
Note that $\pd{g(\vec\theta)^\top}{\vec\theta}$ is a $p \times m$ matrix,
and $\vec\Sigma$ is an $m \times m$ matrix. 
Statistically, $\vec\Sigma$ is related to the covariance matrix, 
$\mv c$ to the correlation between the response and the regressors,
and $s_Y$ to the empirical second moment of the regressand.
Theorem~\ref{thm:Sigma:h} allows us to compute the two key steps of BGD 
{\em without} scanning through the data again, because the quantities 
$(\vec\Sigma, \mv c, s_Y)$ can be computed efficiently in a preprocessing 
step {\em inside the database} as aggregates over the query $Q$. 
We explain this point further below and in the next section.

When $g$ is an identity function, i.e., the model is linear,
as is the case in $\pr$ (and thus $\lr$) model,  
equations~\eqref{eqn:point:eval}
and~\eqref{eqn:gradient} become particularly simple:

\bcor
In a linear model (i.e. $g(\vec\theta)=\vec\theta$), 
\begin{eqnarray}
   J(\vec\theta) &=& \frac 1 2 \vec\theta^\top \vec\Sigma \vec\theta
   - \inner{\vec\theta, \mv c} + s_Y
   +\frac \lambda 2 \norm{\vec\theta}_2^2\label{eqn:point:eval:pr}\\
   \grad J(\vec\theta) &=& \vec\Sigma \vec\theta+
   \lambda\vec\theta-\mv c\label{eqn:gradient:pr}
\end{eqnarray}
Let $\mv d=\grad J(\vec\theta)$. The Armijo condition
$J(\vec\theta-\alpha\mv d)\geq J(\vec\theta)-\frac \alpha
2\norm{\mv d}_2^2$ is equivalent to the following 
\begin{equation}
   \alpha \vec\theta^\top\vec\Sigma\mv d 
   -\frac{\alpha^2}{2}\mv d^\top\vec\Sigma\mv d
      -\alpha \inner{\mv c,\mv d}
   + \lambda \alpha \inner{\vec\theta,\mv d}
   \leq \frac \alpha 2(\lambda\alpha+1)\norm{\mv d}_2^2
   \label{eqn:alternative:armijo}
\end{equation}
\label{cor:Sigma:h}
Lastly,
\begin{equation}
   \grad J(\vec\theta - \alpha \mv d) = (1-\alpha)\mv d - \alpha \vec\Sigma \mv
   d.
   \label{eqn:next:grad}
\end{equation}
\ecor
The significance of~\eqref{eqn:alternative:armijo} is as follows.
In a typical iteration of BGD, we have to backtrack a few times (say $t$
times) for each value of $\alpha$. If we were to recompute
$J(\vec\theta-\alpha\mv d)$ using~\eqref{eqn:point:eval:pr} each time, then
the runtime of Armijo backtracking search is $O(tm^2)$, even after we have
already computed $\mv d$ and $J(\vec\theta)$.
Now, using~\eqref{eqn:alternative:armijo}, we can compute in advance 
the following quantities (in this order): 
$\mv d$, 
$\norm{\vec\theta}_2^2$,
$\vec\Sigma\mv d$, 
$\inner{\mv c, \mv d}$, 
$\inner{\vec\theta, \mv d}$, 
$\mv d^\top\vec\Sigma\mv d$,
$\vec\theta^\top\vec\Sigma\mv d$,
After that, each check for
inequality~\eqref{eqn:alternative:armijo} can be done in $O(1)$-time, for a
total of $O(m^2+t)$-times.
Once we have determined the step size $\alpha$, \eqref{eqn:next:grad}
allows us to compute the next gradient (i.e. the next $\mv d$) in linear
time, because we have already computed $\vec\Sigma \mv d$ for line search.
As we shall see later, with categorical variables time saving from these
simple observations is significant.

To implement BGD, we need to precompute the covariance matrix $\vec\Sigma$ and
the correlation vector $\mv c$ in order to evaluate~\eqref{eqn:gradient}
and~\eqref{eqn:point:eval}. We do not need to compute the second moment $s_Y$
because optimizing $J(\vec\theta)$ is the same as optimizing
$J(\vec\theta)-s_Y$. If all attributes from $Q(D)$ are continuous features,
then $\vec\Sigma=(\sigma_{ij})_{i,j=1}^m$ is a matrix
and $\mv c = (c_i)_{i=1}^m$ is a vector defined more precisely by
\begin{eqnarray}
   \sigma_{ij}&=& \frac{1}{|Q(D)|} \sum_{(\mv x, y)\in Q(D)} h_i(\mv x)h_j(\mv x)
   \label{eqn:sigma:ij}\\
   c_j &=& \frac{1}{|Q(D)|} \sum_{(\mv x,y)\in Q(D)} y\cdot h_j(\mv x).\label{eqn:c:j}
\end{eqnarray}
Here, $h_j$ denote the $j$th component function of the vector-valued function
$h$, and $h_j$ is a multivariate monomial in $\mv x$. Hence, it is easy to see
that both expressions~\eqref{eqn:sigma:ij} and~\eqref{eqn:c:j} are {\sf
Sum-Product} expressions as explained in the Functional Aggregate Queries
framework~\cite{faq}. These $m^2$ aggregates can be computed using known 
algorithms~\cite{faq,SOC16} in time $O(N^{\fhtw})$, where $\fhtw$ is the {\em
fractional hypertree width}~\cite{DBLP:journals/talg/GroheM14} of the input 
query $Q$'s hypergraph $\calH$,
and $N$ is the input database size, for an overall runtime of $O(m^2 N^{\fhtw})$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Tensor representation and computation}
\label{subsec:tensor}

The more interesting, more common, and much more challenging situation is when
some attributes of $Q(D)$ are categorical features. We next explain how we model and
deal with categorical features in the precomputation of $\vec\Sigma$ and $\mv c$.
The main idea can be explained with our running
example~\ref{ex:categorical:features}.

\begin{ex}
In example~\ref{ex:categorical:features},
the matrix $\vec\Sigma$ is of size $8\times 8$ 
instead of $3\times 3$ after one-hot encoding. However, many of those entries are $0$, for instance $\forall \mv x \in Q(D)$:
\begin{eqnarray*}
h_{1,\textsf{vietnam}}(\mv x)  h_{1,\textsf{england}}(\mv x) &=&0\\
h_{1,\textsf{england}}(\mv x)  h_{2,\textsf{vietnam},\textsf{blue}}(\mv x) &=& 0\\
   h_{2,\textsf{vietnam},\textsf{blue}}(\mv x)
   h_{2,\textsf{england},\textsf{blue}}(\mv x) &=& 0\\
   h_{2,\textsf{vietnam},\textsf{blue}}(\mv x)
   h_{2,\textsf{vietnam},\textsf{red}}(\mv x) &=& 0.
\end{eqnarray*}
The reason is that the indicator variables $x_{\textsf{blue}}$ or
$x_{\textsf{england}}$ are like selection clauses 
$x_{\textsf{color}} = \textsf{blue}$
or
$x_{\textsf{country}} = \textsf{england}$.
Thus, we can rewrite an entry $\sigma_{ij}$ as an aggregate over a
more selective query:
\[ 
   \sum_{\mv x \in Q(D)} 
h_{1,\textsf{vietnam}}(\mv x) 
h_{2,\textsf{vietnam},\textsf{red}}(\mv x) 
= \sum_{\phi} x_a^2x_cx_b.
\]
where $\phi := (\mv x \in Q(D) \wedge x_{\textsf{color}} = \textsf{red}\wedge x_{\textsf{country}} = \textsf{vietnam})$.
\end{ex}
Extrapolating straightforwardly, if we were to write $\vec\Sigma$ down in the
one-hot encoded feature space, then
the entries $\sigma_{ij}$ under one-hot encoding got exploded into many entries.
More concretely, $\sigma_{ij}$ is in fact a tensor $\vec\sigma_{ij}$ of dimension
$\prod_{f\in C_i } |\pi_f(Q)| \times \prod_{f\in C_j} |\pi_f(Q)|$, because
\begin{equation}
   \vec\sigma_{ij} = \frac{1}{|Q(D)|} \sum_{(\mv x, y)\in Q(D)} h_i(\mv x)
   \otimes h_j(\mv x)
\label{eqn:sigma:ij:categorical}
\end{equation}
Similarly, $c_j$ in \eqref{eqn:c:j} is a tensor $\mv c_j$ of dimension $\prod_{f\in C_j } |\pi_f(Q)|$ since the monomial $h_j(\mv x)$ is a matrix in the categorical case.

{\bf Sparse tensor representation.}
The dimensionalities of $\vec\sigma_{ij}$ and $\mv c_j$ can be a humongous numbers.
Fortunately, the tensor is very sparse, and a sparse representation 
of it can be computed with {\bf one} aggregate query as the following 
proposition shows.
For any event $E$, let $\mv 1_E$ denote the Kronecker delta, i.e. $\mv 1_{E}=1$
if $E$ holds, and $\mv 1_{E} = 0$ otherwise. 
Recall that the input query $Q$ has hypergraph $\calH= (\calV,\calE)$,
and there is an input relation $R_F$ for every hyperedge $F \in \calE$.


\bprop
The tensor $\vec\sigma_{ij}$ can be sparsely represented by an aggregate query
with group-by attributes $C_i \cup C_j$. 
In the $\faq$-framework, the query is expressed as a {\sf Sum-Product} query 
with free (i.e., group-by) variables:
\begin{equation}
   \varphi(\mv x_{C_i\cup C_j}) = 
   \sum_{x_f : f \notin C_i\cup C_j} \prod_{f \notin C_i \cup C_j}
   x_f^{e_{i}(f)+e_{j}(f)} \prod_{F\in \calE} \mv 1_{\pi_F(\mv x) \in R_F}.
   \label{eqn:faq}
\end{equation}
Similarly, the tensor $\mv c_j$ can be sparsely represented by an aggregate
query with group-by attributes $C_j$, which is expressed as the 
{\sf Sum-Product} query
\begin{equation}
   \varphi(\mv x_{C_j}) = 
   \sum_{x_f : f \notin \cup C_j \cup \{y\}} 
   y \prod_{f \cup C_j} x_f^{e_{j}(f)} \cdot \prod_{F\in \calE} \mv 1_{\pi_F(\mv x) \in R_F}.
   \label{eqn:faq2}
\end{equation}
\eprop

\begin{ex}\label{ex:store:city}
   Consider the query $Q$ in~\eqref{eqn:running:Q}, where the set of features is
   $\{\textsf{sku, store, day, color, quarter, city, country}\}$
   and  \textit{unitSold} is the response variable. In this query $n=7$, and thus
   for a $\pr_2$ model we have $m=1+7+7^2=57$ parameters. Consider two indices $i$ and $j$ to the component functions of $g$ and $h$, where 
   $i = (\textsf{store, city})$ and $j = (\textsf{city})$.
   Suppose the query result states that the retailer has $N_s$ stores in $N_c$ countries. Then, the full dimensionality of
   the tensor $\vec\sigma_{ij}$ is $N_s \times N_c^2$, because by definition
   it was defined to be
   \begin{equation} \vec\sigma_{ij} := \frac{1}{|Q(D)|}\sum_{(\mv x,y)\in Q(D)} 
        \underbrace{\mv x_{\textsf{store}} \otimes 
        \mv x_{\textsf{city}}}_{h_i(\mv x)} \otimes 
        \underbrace{\mv x_{\textsf{city}}}_{h_j(\mv x)}.
        \label{eqn:store:city}
   \end{equation}
   Recall that $\mv x_{\textsf{store}}$ and $\mv x_{\textsf{city}}$ are both
   indicator vectors. Consequently, the above tensor has the following
   straightforward interpretation: for every triple $(s,c_1,c_2)$, where $s$
   is a store and $c_1$ and $c_2$ are cities, this triple entry of the
   tensor counts the number of data points $(\mv x, y) \in Q(D)$ for this particular
   combination of store and cities (divided by $1/|Q(D)|$). It is clear  
   that most of these $(s,c_1,c_2)$-entries are $0$. For example, if 
   $c_1\neq c_2$ then the count is zero. Thus, we can concentrate on computing
   entries of the form $(s,c,c)$:

   \texttt{SELECT s, c, count(*) FROM Q GROUP BY s, c;}

   Better yet, since {\sf store} functionally determines {\sf city}, the number
   of entries in the output of the above query is bounded by $N_s$. 
   Using database relations to represent sparse tensor results 
   in a massive amount of space saving.
\end{ex}

{\bf Computing $\vec\Sigma$ and $\mv c$.} We employ three orthogonal ideas 
to compute the queries~\eqref{eqn:faq} and~\eqref{eqn:faq2} efficiently.

First, our $\faq$~\cite{faq} and $\fdb$~\cite{SOC16} frameworks are designed to compute such aggregates over feature extraction queries, which are wider than traditional OLAP queries.

\bprop
Let $\faqw(i,j)$ denote the {\em $\faq$-width} of the query corresponding to $\vec\sigma_{ij}$, and $S(i,j)$ denote the size of the sparse representation, i.e., the number of tuples, used to represent the tensor $\sigma_{ij}$. Then, the worst-case runtime for computing $\vec\Sigma$ and $\mv c$ is  
$O\left( \sum_{i,j\in [m]} ( N^{\faqw(i,j)} + S(i,j) )\log N \right)$. 
\eprop

The notion of $\faq$-width is beyond the scope of this paper. The tensor~\eqref{eqn:store:city} has $\faqw(i,j)=1$ and $S(i,j) = O(N)$.

Second, we exploit the observation that in the computation of $\vec\Sigma$ many {\em distinct} tensors $\vec\sigma_{ij}$ have {\em identical} sparse representations.  Consider, for example, the tensor $\vec\sigma_{ij}$ from Example~\ref{ex:store:city} corresponding to $i = (\textsf{store, city})$ and $j = (\textsf{city})$. Following equation~\eqref{eqn:faq}, all of the following tensors have the exact same 
sparse representation:
$(i,j) \in \{
(({\sf store, city}), {\sf city}),$
$(({\sf store, store}), {\sf city}),$
$(({\sf store, city}), {\sf store}),\ldots\}$.
There are $12$ tensors sharing this particular sparse representation.
\nop{
% (1,sc), (sc,1), 
% (s, c), (c, t)
% (ss, c), (c, ss), (s, sc), (sc, s), 
% (cc, s), (s, cc), (c, sc), (sc, c).
}
Formula~\eqref{eqn:faq} tells us which tensors share the same representation:
The output function $\varphi$ is identified by the tuple $(C_i \cup C_j, (e_i(f)+e_j(f))_{f \in V-C_i\cup C_j})$. Tensors sharing the same tuple will share the same sparse representation. In the tuple, $C_i \cup C_j$ identify the set of group-by variables, and the exponents $(e_i(f)+e_j(f))_{f \in V-C_i\cup C_j}$ specify which function we want to compute for those group-by variables.

Third, we employ a sparse representation of tensors in the parameter space. We need to evaluate the component functions of $g$, which are polynomial. In the $\fama_2^r$ example,  for instance, we evaluate expressions of the form
\begin{equation}
   g_{\textsf{store, city}}(\vec\theta) = 
   \sum_{\ell=1}^r 
   \vec\theta^{(\ell)}_{\textsf{store}} \otimes
   \vec\theta^{(\ell)}_{\textsf{city}}.
   \label{eqn:g:store:city}
\end{equation}
The result is a $2$-way tensor whose CP-decomposition (a sum of rank-$1$ tensors) is already given! There is no point in materializing the result of $g_{\textsf{store, city}}(\vec\theta)$ and we instead keep it as is. If we were to materialize it, we would end up with an $\Omega(N^2)$-sized result for absolutely no gain in computational  and space complexity, while the space complexity of the CP-decomposition is only $O(N)$. This is a prime example of factorization of the parameter space.

{\bf Point evaluation and gradient computation.}
Finally, we explain how to evaluate the expressions~\eqref{eqn:point:eval} 
and~\eqref{eqn:gradient} with our sparse tensor representations.
There are two aspects of our solution worth spelling out:
(1) how to multiply two tensors, e.g., $\vec\sigma_{ij}$ and $\vec\theta_j$, and (2) how to exploit that some tensors have the same representation to speed up the point evaluation and gradient computation.

To answer question (1), we need to know the intrinsic dimension of the tensor
$\vec\sigma_{ij}$. In order to compute $\vec\Sigma g(\vec\theta)$ in
Example~\ref{ex:store:city}, we need to multiply $\vec\sigma_{ij}$ with
$g_j(\vec\theta)$ for $i = (\textsf{store, city})$ and $j = (\textsf{city})$. In
a linear model, $g_j(\vec\theta) = \vec\theta_j = \vec\theta_{\textsf{city}}$.
In this case, when computing $\vec\sigma_{ij} \vec\theta_{\textsf{city}}$ we
marginalize away one {\sf city} dimension of the tensor, while keeping the other two dimensions {\sf store, city}. This is captured by the following query:
\begin{align*}
&\texttt{SELECT store, city, sum}(\vec \sigma_{i,j}.\texttt{val} * \vec \theta_j.\texttt{val})\\
&\texttt{FROM } \vec \sigma_{i,j}, \vec \theta_j \texttt{ WHERE } \vec
   \sigma_{i,j}.\texttt{city} = \vec \theta_j.\texttt{city}\\
&\texttt{GROUP BY store, city;}
\end{align*}
where the tensors $\vec \sigma_{i,j}$ and $\vec \theta_j$ map $(\textsf{store, city})$ and respectively $(\textsf{city})$ to aggregate values. In words, $\vec\sigma_{ij} g_j(\vec\theta)$ is computed by a group-by aggregate query where the group-by variables are precisely the variables in $C_i$.

\nop{
In LogiQL,
the query is
\begin{verbatim}
result_i[store, city] = v 
   <- agg<<v = total(z)>>
         sigma_ij[store, city] = x,
         theta_j[city] = y, z = x*y.
\end{verbatim}
}

For the second question, we use the CP-decomposition of the parameter space as discussed earlier. Suppose now we are looking at the $\vec\sigma_{ij}$ tensor where  $i = (\textsf{city})$ and $j = (\textsf{store, city})$. Note that this tensor has the identical representation as the above tensor, but it is a {\em different} tensor. In a $\fama_2^r$ model, we would want to multiply this tensor with the component function $g_j(\vec\theta)$ defined in~\eqref{eqn:g:store:city} above. We do so by multiplying it with each of the terms $\vec\theta^{(\ell)}_{\textsf{store}} \otimes \vec\theta^{(\ell)}_{\textsf{city}}$, one by one for $\ell = 1, \dots, r$, and then add up the result. Multiplying the tensor $\vec\sigma_{ij}$ with the first term $\vec\theta^{(1)}_{\textsf{store}} \otimes \vec\theta^{(1)}_{\textsf{city}}$ corresponds precisely to the following query:

\begin{align*}
&\texttt{SELECT city, sum}(\vec\sigma_{i,j}.\texttt{val} * \vec\theta^{(1)}_{\texttt{store}}.\texttt{val} * \vec\theta^{(1)}_{\texttt{city}}.\texttt{val})\\
&\texttt{FROM } \vec\sigma_{i,j}, \vec\theta^{(1)}_{\texttt{store}}, \vec\theta^{(1)}_{\texttt{city}}\\
&\texttt{WHERE } \vec\sigma_{i,j}.\texttt{city} =  \vec\theta^{(1)}_{\texttt{city}}.\texttt{city} \texttt{ AND }\\
& \qquad \quad \vec\sigma_{i,j}.\texttt{store} =  \vec\theta^{(1)}_{\texttt{store}}.\texttt{store}\\
&\texttt{GROUP BY city;}
\end{align*}
where the tensors $\vec\sigma_{i,j}$, $\vec\theta^{(1)}_{\textsf{city}}$, and
$\vec\theta^{(1)}_{\textsf{store}}$ map $(\textsf{store, city})$, $(\textsf{city})$, and respectively 
$(\textsf{store})$ to aggregate values.

\nop{
\begin{verbatim}
result_1[city] = v <- agg<<v = total(z)>>
                        sigma_ij[store, city] = x, 
                        theta_store_1[store] = y,
                        theta_city_1[city] = z, 
                        t = x*y*z.
\end{verbatim}
}

Finally, to answer question (2), note that for the same column $j$ (i.e., the same component function $g_j(\vec\theta)$), there can be multiple tensors $\vec\sigma_{ij}$ which have identical sparse representation. (This is especially true in degree-$2$ models.)  In such cases, we have queries with identical from-where blocks but different select-group-by clauses, because the tensors have different group-by variables. Nevertheless, all such queries can share computation as we can compute the from-where clause once for all of them and then scan this result to compute each specific tensor.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{FD-based dimensionality reduction}
\label{sec:fds}

Consider a query $Q$ in which {\sf country} and {\sf city} are two attributes
representing features.
For simplicity, assume that there are only two countries ``vietnam'' and
``england'', and $5$ cities ``saigon'', ``hanoi'', ``london'',
``leeds'', and ``bristol''.
Under one-hot encoding, the corresponding features are of the form
$x_{\vietnam}$,
$x_{\text{\sf england}}$,
$x_{\saigon}$,
$x_{\hanoi}$,
$x_{\textsf{london}}$,
$x_{\textsf{leeds}}$,
$x_{\textsf{bristol}}$.
Since {\sf city} $\to$ {\sf country} is an FD, we know that, for a given tuple
$\mv x$ in the query result, the following identities hold:
\begin{eqnarray}
   x_{\vietnam} &=& x_{\saigon} + x_{\hanoi}\label{eqn:x:vietnam}\\
   x_{\england} &=&
   x_{\textsf{london}}+x_{\textsf{leeds}}+x_{\textsf{bristol}}\label{eqn:x:england}.
\end{eqnarray}
The first identity states that if a tuple in the query result has $\vietnam$ as the
value for {\sf country} ($x_{\vietnam}=1$), then it can only have as value for
city either $\saigon$ ($x_{\saigon}=1$ and $x_{\hanoi}=0$) or $\hanoi$ ($x_{\hanoi}=1$
and $x_{\saigon}=0$). The second identity has a similar
explanation\footnote{Composite FDs lead to more complex identities. For
instance, the FD {\sf (guest, hotel, date)} $\to$ {\sf room} leads to the
identity $x_{\textsf{room}} = \sum
x_{\textsf{guest}}x_{\textsf{hotel}}x_{\textsf{date}}$. 
We do not explore such polynomial correlations in this paper.}.

The linear relationship only holds if both variables are categorical. An FD on categorical and continuous features cannot be ``linearized'' this way, e.g., the FD {\sf SSN} $\to$ {\sf salary}, where SSN is categorical but salary is continuous.

Where do these identities come from? We can extract in a preprocessing step from the database a relation of the form $R(\city, \country)$ with $\city$ as a primary key. How do we express the identities such as~\eqref{eqn:x:vietnam}
and~\eqref{eqn:x:england} in a formal manner
in terms of the input vectors 
$\mv x_{\textsf{city}}$ and $\mv x_{\textsf{country}}$?  
Suppose there are $N_\city$ cities
and $N_\country$ countries. 
The predicate $R(\city, \country)$ can be
modeled mathematically with an $N_\country \times N_\city$ 
matrix $\mv R$: if $\mv x_\city$ is an indicator vector for {\sf saigon},
then $\mv R\mv x_\city$ is an indicator for {\sf vietnam}.\footnote{The
predicate is a sparse representation of the matrix!} 
In this language,
the above identities are written as $\mv x_\country = \mv R\mv x_\city$.
For example, in the above particular example $N_\city = 5$, $N_\country=2$,
and
\[ \mv R = \begin{matrix}
   & \text{saigon}&\text{hanoi}&\text{london}&\text{leeds}&\text{bristol}\\
   &1&1&0&0&0&\text{viet}\\
   &0&0&1&1&1&\text{eng}.
\end{matrix}
\]
This relationship suggests a natural but powerful technique: we may 
replace any occurrence of statistics $\mv x_t$ by its functionally 
determining quantity $\mv x_c$. Since these quantities are present only in
loss $\calL$ via inner products
$\langle g(\mv x), h(\vec\theta) \rangle$, such replacements result in
a (typically) linear reparameterization of the loss. What happens next is less obvious,
due to the presence of nonlinear penalty function $\Omega$.
Depending on the specific structure of FDs
and the choice of $\Omega$, it turns out that 
many parameters associated with redundant statistics, which do not affect
the loss $\calL$, can be optimized out directly with respect to the transformed 
$\Omega$ penalty. Our reparameterization technique thus entails a number of 
benefits: (1) the number of required precomputations
is reduced drastically, (2) the transformed parameter space is also reduced in 
dimensions, which potentially helps to speed up the convergence in the optimization phase.

The remainder of this subsection is a gentle introduction of our idea in the
presence of {\em one} simple FD. A general development of this technique
will be presented in its full glory in the sequel, by accounting for more general
FD structures in the context of $\pr$ and $\fama$ learning problems.
Consider a query $Q$ in which
$\city$ and $\country$ are two of the categorical features, functionally
determine one another via a matrix $\mv R$ such that $\mv R \mv x_\city = \mv
x_\country$ for all $\mv x = (\cdots, \mv x_\city,\mv x_\country, \cdots) \in Q$. 
We use this linear correlation to eliminate $\mv x_\country$ from the model as
follows.
\begin{eqnarray*}
   && \inner{g(\vec\theta),h(\mv x)} = \inner{\vec\theta,\mv x}\\
   &=& \sum_{j\notin \{\city,\country\}}\inner{\vec\theta_j,\mv x_j}+
   \inner{\vec\theta_\city,\mv x_\city}
   + \inner{\vec\theta_\country,\mv x_\country}\\
   &=& \sum_{j\notin \{\city,\country\}}\inner{\vec\theta_j,\mv x_j}+
   \inner{\vec\theta_\city,\mv x_\city} + \inner{\vec\theta_\country, \mv R \mv x_\city}\\
%   &=& \sum_{j\notin \{\city,\country\}}\inner{\vec\theta_j,\mv x_j}+
%   \inner{\vec\theta_\city,\mv x_\city} + \inner{\mv R^\top\vec\theta_\country, \mv x_\city}\\
   &=& \sum_{j\notin \{\city,\country\}}\inner{\vec\theta_j,\mv x_j}+
   \inner{\underbrace{\vec\theta_\city + \mv R^\top
   \vec\theta_\country}_{\vec\gamma_\city},\mv x_\city}
\end{eqnarray*}
Reparameterize the model by defining $\vec\gamma = (\vec\gamma_j)_{j \in
V-\{\country\}}$, and two new functions $\overline g : \R^{n-1} \to \R^{n-1}$,
$\overline h : \R^n \to \R^{n-1}$ by
\begin{eqnarray}
   \vec\gamma_j &=& 
   \begin{cases}
   \vec\theta_j & j \notin \{ \city, \country\}\\
   \vec\theta_\city +\mv R^\top \vec\theta_\country &  j = \city.
   \end{cases}\\
   \overline g(\vec\gamma) &=& \vec\gamma\\
   \overline h_j(\mv x) &=& \mv x_j, \ j \neq \city.
\label{eqn:var:change:1}
\end{eqnarray}
(Note again that there is no $\vec\gamma_\country$.) Then, we can rewrite
$J(\vec\theta)$ in terms of $\vec\gamma$:
\begin{align*} 
   J(\vec\theta) &=  \frac{1}{2|Q|}\sum_{(\mv x,y)\in Q}
   \inner{g(\vec\theta),h(\mv x)} 
   + \frac\lambda 2 \norm{\vec\theta}_2^2\\
   &= \frac{1}{2|Q|}\sum_{(\mv x,y) \in Q} \inner{\overline g(\vec\gamma), \overline h(\mv x)}\\
   &
   + \frac\lambda 2 \left( \sum_{j\neq \city} \norm{\vec\gamma_j}^2 
   + \norm{\vec\gamma_\city - \mv R^\top\vec\theta_\country}^2
   + \norm{\vec\theta_\country}^2
   \right)
\end{align*}
Note how $\vec\theta_\country$ has disappeared from the loss term, but it still
remains in the penalty term. Since the penalty is data-independent, $\vec\theta_\country$
can be optimized out easily. The partial derivative of $J$ with respect
to $\vec\theta_\country$:
\begin{equation}
   \frac{2}{\lambda} \pd{J}{\vec\theta_\country} 
   = \mv R (\mv R^\top \vec\theta_\country- \vec\gamma_\city) +
   \vec\theta_\country \label{eqn:pd:10}
%   \frac 1 2 \pd{J}{\vec\gamma_\city} 
%   &=& \vec\gamma_\city-\mv R^\top \vec\theta_\country\label{eqn:pd:11}
\end{equation}
By setting~\eqref{eqn:pd:10} to $0$ we obtain
$\vec\theta_\country$ in terms of $\vec\gamma_\city$:
$\vec\theta_\country = {\mv R (\mv I + \mv R^\top \mv R)^{-1}}
\vec\gamma_\city$. ($\mv I$ is the identity matrix.) 
So, $J$ can be expressed completely in terms of 
$\vec\gamma$, its gradient with respect to $\vec\gamma$ is also
available:
\begin{align*}
   J(\vec\theta) &=
   \frac{1}{2|Q|}\sum_{(\mv x,y) \in Q} \inner{\overline g(\vec\gamma), \overline h(\mv x)}\\
   &
   + \frac\lambda 2 \left( \sum_{j\neq \city} \norm{\vec\gamma_j}^2 
   + \inner{(\mv I + \mv R^\top \mv R)^{-1}\vec\gamma_\city,\vec \gamma_\city}
   \right),\\
   \frac 1 2 \pd{\norm{\vec\theta}_2^2}{\vec\gamma_j} 
   &=
   \begin{cases}
      \vec\gamma_j & j \neq \city\\
      \left( \mv I + \mv R^\top \mv R) \right)^{-1}
      \vec\gamma_\city & j = \city.
   \end{cases}
\end{align*}
The gradient of the loss term is computed using the matrix $\overline{\vec\Sigma}$
and the vector $\overline{\mv c}$ with respect to the dimensionality-reduced pair
$(\overline g,\overline h)$.
The matrix $(\mv I + \mv R^\top\mv R)$ is a rank-$N_\country$ update to the identity
matrix, strictly positive definite and thus invertible. (The inverse can be obtained
using the Sherman-Morrison-Woodbury identity~\cite{MR997457}.) 
It is important to keep in mind the database interpretation of the product $\mv
R^\top \mv R$: this is an $N_\city \times N_\city$ binary matrix whose rows and columns 
are indexed by cities, where there is a $1$ at entry $(c_1,c_2)$ iff both cities
belong to the same country. It should be obvious that 
-- using a ternary predicate with two keys and one value --
a sparse representation of $(\mv I + \mv R^\top\mv R)$ can be computed using 
database queries.

\subsection{Reparameterization and optimization with general FD structures}

The variable elimination and reparameterization techniques described above
will be developed in full generality, which help to simplify and substantially 
speedup the training of 
$\pr$ and $\fama$ under an arbitrary set of simple FDs. 
To formalize general FD structures, consider a query $Q$ in which there are
$k$ groups of disjoint categorical features $F_1,\dots,F_k$. In group $i$, there
is a feature $f_i$ which functionally determines the remaining features in the
group. We write $F_i = \{f_i\} \cup S_i$, and $f_i \to S_i$ is an FD. For
example, in a typical data modeling query we see at $\LB$'s retailer customer, 
we have $k=3$ groups
(among other attributes): in the first group we have {\sf day} $\to$ {\sf week}
$\to$ {\sf month} $\to$ {\sf quarter} $\to$ {\sf year}, and thus $f_1$ = {\sf
day} and $S_1$ = $\{$ {\sf week, month, quarter, year} $\}$. In the second
group, $f_2$ = {\sf sku} and $S_2 = \{$ {\sf type, color, size, ...}$\}$ (this is a
rather large group). In the third group $f_3 = $ {\sf store} and
$C_3 = \{$ {\sf city, country, region, continent} $\}$.
We shall refer to these as 
{\em groups of simple FDs} in the statements of theorems below.
Similar to the setting above, for each feature $c \in S_i$, let $\mv R_c$ denote
the matrix for which $\mv x_c = \mv R_c \mv x_{f_i}$.
For the sake of brevity, we also define a matrix $\mv
R_{f_i} = \mv I_{f_i}$ (the identity matrix of dimension equal to the active
domain size of attribute $f_i$); this way the equality 
$\mv R_c\mv x_{f_i} = \mv x_c$ holds for every $c \in F_i$.

\bdefn
Given a pair of functions $g$ and $h$ in our problem setting.
%for a linear model such as $\lr$ and $\pr$. %Recall that in such model $g(\vec\theta) = \vec\theta$. 
Define
\[ T := \{ j \in [m] \suchthat C_j \cap (S_1 \cup \dots \cup S_k) \neq \emptyset
  \} \]
(In words, $T$ is the set of component functions of $h$ containing at least one
functionally determined variable.)
The group of simple FDs induces an {\em FD-reduced pair} of functions 
$\overline g : \R^{m-|T|} \to \R^{m-|T|}$ and 
$\overline h : \R^{n} \to \R^{m-|T|}$ defined as follows. 
The component functions of $\overline h$ are obtained from 
from the component functions of $h$ by removing all component functions $h_j$
for $j \in T$. Similarly, 
$\overline g$ is obtained from $g$ by removing all component functions 
$g_j$ for which $j \in T$. 
Naturally, define the covariance matrix $\overline{\vec\Sigma}$ and the correlation vector
$\overline{\mv c}$ as in~\eqref{eqn:sigma} and~\eqref{eqn:c}, but with respect to $\overline h$.
\edefn

The following theorem is established for $\lr$ learning.

\bthm
Consider a $\lr$ model with $k$ groups of simple FDs $F_i = \{f_i\}\cup S_i$,
$i \in [k]$. Let $\vec\theta=(\vec\theta_i)_{i\in V}$ be the original
parameters. Define the following reparameterization:
\[
   \vec\gamma_w = 
   \begin{cases}
      \vec\theta_w & w \in V - \{f_1,\dots,f_k\}\\
      {\sum_{c\in F_i}\mv R^\top_c \vec\theta_c}& w=f_i, i\in [k].
     \end{cases}
\]
Then, minimizing $J(\vec\theta)$ is equivalent to minimizing the
function %$\overline J(\vec\gamma)$:
$\overline J(\vec\gamma) := \frac 1 2 \vec\gamma^\top \overline{\vec\Sigma} \vec\gamma
- \inner{\vec\gamma,\overline{\mv c}} + \frac\lambda 2 \Omega(\vec\gamma),$
where
$\Omega(\vec\gamma) := 
\sum_{w \in V\setminus F}\norm{\vec\gamma_w}^2+\sum_{i=1}^k\inner{\gamma_{f_i},\mv B_i^{-1}\gamma_{f_i}}
$, and matrix $B_i$ for each $i \in [k]$ is given by
\begin{equation}
   \mv B_i := \sum_{c\in F_i}\mv R^\top_c \mv R_c.\label{eqn:B:i}
\end{equation}
%$\mv B_i^{-1}$ is invertible because it is a series of
%rank-$1$ updates to a symmetric positive definite matrix. Furthermore, as
%aforementioned, (a sparse representation of)
%the matrix $\mv B_i$ can be computed using aggregate queries to the database.
\label{thm:fd:lr}
\ethm

\noindent {\bf Remarks} According to the proof of the theorem,
$\overline J$ is defined with respect to the FD-reduced pair of
functions $\overline{g}, \overline{h}$ and a reduced parameter
space of $\vec\gamma$. Its gradient is very simple to compute, due
the fact that
\begin{eqnarray}
   \frac 1 2 \pd{\Omega(\vec\gamma)}{\vec\gamma_w} &=& 
   \begin{cases}
      \vec\gamma_w & w \notin \{f_i\}_{i=1}^k\\
      {\mv B_i^{-1} \vec\gamma_{f_i}}& w = f_i
   \end{cases}
\end{eqnarray}
Moreover, once a minimizer $\vec\gamma$ of $\overline J$ is obtained,
we can compute a minimizer $\vec\theta$ of $J$ by setting
\[
   \vec\theta_w =
   \begin{cases}
      \vec\gamma_w & w \in V\setminus F\\
      \mv R_w \mv B_i^{-1} \vec\gamma_{f_i} & w \in F_i, i \in [k].
   \end{cases}
\]

We proceed to higher degree models. Our method works in general, but we
will only present the results for $\pr$ and $\fama$ of degree $2$, partly because
in practice one rarely train models of higher degrees (there are too many
parameters).
% and also because the  mathematics is a bit simpler to state within
%the space limitation. 
We start with the $\pr$ model of degree $2$. With categorical features, 
we do not need the parameters
$\vec\theta_{ww}$ if $w$ is a categorical feature, because the term
simplifies to be linear any how:
$\inner{\vec\theta_{ww}, \mv x_w \otimes \mv x_w} =
   \inner{\diag(\vec\theta_{ww}), \mv x_w},
$
where -- abusing notation -- we use $\diag(\mv A)$ to denote the vector
consisting of diagonal entries from the matrix $\mv A$.
\iffalse
some of 
the second order parameters are simplified in the following sense:
\bi
\item First, 
we do not need the parameters
$\vec\theta_{ww}$ if $w$ is a categorical feature, because the term
simplifies to be linear any how:
$\inner{\vec\theta_{ww}, \mv x_w \otimes \mv x_w} =
   \inner{\diag(\vec\theta_{ww}), \mv x_w},
$
where -- abusing notation -- we use $\diag(\mv A)$ to denote the vector
consisting of diagonal entries from the matrix $\mv A$.
\item Second, If $c, t \in F_i$ belong  to the same FD group, then many of the entries in the
$\vec\theta_{ct}$ matrix are $0$: 
we can set $\theta_{ct}=0$ whenever
there does {\em not} exist ${f_i}$ for which $f_i\to c$ and $f_i \to t$.
This is because, in the model because, for such entries, 
$\theta_{{f_i}t}x_{f_i}x_t=0$.\footnote{E.g.,
$\theta_{\text{\sf vietnam},\text{\sf london}}x_{\text{\sf vietnam}}
x_{\text{\sf london}}=0$} 
Setting those entries to $0$ is equivalent to ``selecting out'' some entries
of the matrix $\vec\theta_{ct}$ to be real parameters, while keeping the rest
at $0$. This selection can be modeled with the vector
$\diag(\mv R_c^\top \vec\theta_{ct}\mv R_t)$,
which consists only of the entries of $\vec\theta_{ct}$ that were not
set to $0$.\footnote{Here $\diag(\mv A)$ denote the vector consisting of diagonal
entries of $\mv A$}
This observation means
that among the attributes in $F_i$ there are only a linear number of parameters
instead of quadratic as the degree of $\pr^2$ might indicate.
 \item Third, consider the case when $(c,t) \in F_i \times F_j$, $i\neq j \in
[k]$.
WLOG we can assume we can set $\theta_{ct}=0$ when there are no $f_i,f_j$ for 
which $f_i \to c$ and $f_j \to t$.
Similar to the previous bullet, the zeroing out is modeled with the matrix
$\mv R_c^\top \vec\theta_{ct}\mv R_t$.
\ei
\fi

There is also a degree-$2$ analog of the matrices $\mv R_c$ defined earlier.
For any pair $\{c,t\} \in F_i$, let $\mv R_{ct}$ denote the binary
matrix whose $j$th column is the tensor product of the $j$th column of $\mv R_c$
and the $j$th column of $\mv R_t$.\footnote{Formally, $\mv R_{ct} := \mv R_c
\star \mv R_t$, where $\star$ denotes the Khatri-Rao
product where we partition the two matrices by their columns.} Define the matrix
\begin{equation}
   \mv A_i := \sum_{c\in F_i}\mv R^\top_c \mv R_c + \sum_{ct \in \binom{F_i}{2}} \mv R_{ct}^\top\mv R_{ct}, \label{eqn:A:i}
\end{equation}
then this matrix can also be computed using database queries just as $\mv B_i$.
Let $\mv v$ be any vector, we use 
$\DIAG(\mv v)$ to denote the matrix whose diagonal entries are $\mv v$. 

\bthm
Consider a $\pr$ model of degree $2$
with $k$ groups of simple FDs $F_i = \{f_i\}\cup S_i$,
$i \in [k]$. Let $\vec\theta=(\vec\theta_i)_{i\in V}$ be the original
parameters, and $F = \cup_{i\in [k]}F_i$. 
Define the following reparameterization:
\begin{align}
   \vec\gamma_w &= \begin{cases}
      \vec\theta_w & w \in V \setminus F\\
      \displaystyle{\sum_{c\in F_i}\mv R^\top_c \vec\theta_c + \sum_{\{c,t\}\in \binom{F_i}{2}}
\diag\left( \mv R_c^\top \vec\theta_{ct}\mv R_t\right)} &
      \substack{w={f_i}\\ i\in [k]}.
\end{cases}\\
%   \vec\gamma_{f_i}^{ct} &=& \vec\theta_{f_i}^{ct} \ \ \ \ \{c,t\} \in \binom{F_i}{2}, i \in [k]\\
\vec\gamma_{tw} &= 
\begin{cases}
   \vec\theta_{tw} & \{t,w\}\subseteq V\setminus F\\
   \sum_{c\in F_i}\mv R^\top_{c} \vec\theta_{cw} & t=f_i, w \notin F\\
   \displaystyle{\sum_{(c,t) \in F_i\times F_j} \mv R^\top_{c} \vec\theta_{ct} \mv R_{t}  } & \{ t,w\} = \{f_i,f_j\}.
\end{cases}
%   \vec\gamma_{f_if_j}^{ct} &=& \vec\theta_{f_if_j}^{ct} \ \ \ \ (c,t) \in F_i \times F_j - \{(f_i,f_j)\}
\end{align}
Then, minimizing $J(\vec\theta)$ is equivalent to minimizing the
function %$\overline J(\vec\gamma)$:
$\overline J(\vec\gamma) := \frac 1 2 \vec\gamma^\top \overline{\vec\Sigma} \vec\gamma
- \inner{\vec\gamma,\overline{\mv c}} + \frac\lambda 2 \Omega(\vec\gamma),$
where
\begin{multline*}
   \Omega(\vec\gamma) := 
   \sum_{w \notin F}\norm{\vec\gamma_w}^2 + 
       \sum_{\substack{c \notin F\\ t\notin F}} \norm{\vec\gamma_{ct}}^2 +
       \sum_{i=1}^k \inner{\vec\gamma_{f_i},\mv A_i^{-1}\vec\gamma_{f_i}} +\\
       \sum_{\substack{i\in [k]\\ w\notin F}}\inner{\vec\gamma_{f_iw},\mv B_i^{-1}\vec\gamma_{f_iw}}
   + \sum_{ij \in \binom{[k]}{2}} \inner{\mv B_i^{-1} \vec\gamma_{f_if_j}, \vec\gamma_{f_if_j} \mv B_j^{-1}}
\end{multline*}
\label{thm:fd:pr2}
\ethm

\noindent {\bf Remarks} We add some details about this theorem (the proof is deferred
to the \cite{NNOS2017}~Appendix).
$\overline J$ is optimized with respect to the reduced parameter space of $\vec\gamma$.
The gradient of $\overline J$ is very simple to compute, by noticing that
\begin{eqnarray}
   \frac 1 2 \pd{\norm{\vec\theta}^2}{\vec\gamma_w} &=&
   \begin{cases}
      \vec\gamma_w & w \notin F\\
      {\mv A_i^{-1} \vec\gamma_{f_i}}& w = f_i
   \end{cases}\\
   \frac 1 2\pd{\norm{\vec\theta}^2}{\vec\gamma_{tw}} &=&
   \begin{cases}
      \vec\gamma_{tw}& \{t,w\} \cap \{f_i\}_{i=1}^k = \emptyset\\
      \displaystyle{\mv B_i^{-1} \vec\gamma_{f_iw}}& t=f_i,w\notin F\\
      \mv B_i^{-1} \vec\gamma_{f_if_j} \mv B_j^{-1} & \{ t,w\} = \{f_i,f_j\}
   \end{cases}
\end{eqnarray}
Moreover, once a minimizer $\vec\gamma$ of $\overline J$ is obtained, we can easily
achieve a minimizer $\vec\theta$ of $J$ by setting
\begin{eqnarray*}
   \vec\theta_w &=& 
   \begin{cases}
      \vec\gamma_w & w \in V\setminus F\\
      \mv R_w \mv A_i^{-1} \vec\gamma_{f_i} & w \in F_i, i \in [k]\\
   \end{cases}\\
   \vec\theta_{ct} &=& \mv R_c \DIAG(\mv A_i^{-1} \vec\gamma_{f_i}) \mv R_t, \qquad \qquad \forall \{c,t\} \in \binom{F_i}{2}\\
   \vec\theta_{cw} &=& 
   \begin{cases}
      \vec\gamma_{cw} & w \in V\setminus F\\
      \mv R_c\mv B_i^{-1}\vec\gamma_{f_iw}, & c \in F_i, w \notin F, i\in [k]
   \end{cases}\\
   \vec\theta_{ct} &=& \mv R_c \mv B_i^{-1}\vec\gamma_{f_if_j}\mv B_j^{-1} \mv R_t^\top \qquad ct \in F_i\times F_j.
\end{eqnarray*}

Finally, we turn our attention to $\fama$ of degree 2.
\bthm
Consider the $\fama$ model of degree $2$, rank $k$,
with $k$ groups of simple FDs $F_i = \{f_i\}\cup S_i$,
$i \in [k]$. Let $\vec\theta=(\vec\theta_i)_{i\in V}$ be the original
parameters, and $F = \cup_{i\in [k]}F_i$. 
For any $i \in [k]$, define 
\[ \vec\beta_{f_i} := 
\sum_{\ell=1}^r \sum_{\{c,t\} \in \binom{F_i}{2}} 
\mv R^\top_c\vec\theta_c^{(\ell)}\circ \mv R_t^\top \vec\theta_t^{(\ell)}
\]
Define the following reparameterization:\footnote{
Note that there is no $\vec\gamma_c$ for $c \in S_i$, but there is
$\vec\gamma^{(\ell)}_c$ for $c \in S_i$.}
\begin{eqnarray*}
   \vec\gamma_w &=& {\begin{cases}
      \vec\theta_w & w\notin f\\
      \displaystyle{ \vec\theta_{f_i} + \sum_{c\in S_i}\mv R_c^\top\vec\theta_c + \vec\beta_{f_i}} & w = f_i, i \in [k].
   \end{cases}}\\
   \vec\gamma^{(\ell)}_w &=&
   \begin{cases}
      \vec\theta^{(\ell)}_w & w \notin\{f_1,\dots,f_k\} \\ %\notin F = S\cup \{f\}\\
      \vec\theta^{(\ell)}_{f_i} + \sum_{c\in S_i}\mv R_c^\top \vec\theta^{(\ell)}_c & w=f_i, i \in [k]
   \end{cases}
\end{eqnarray*}
Then, minimizing $J(\vec\theta)$ is equivalent to minimizing the
function %$\overline J(\vec\gamma)$:
$\overline J(\vec\gamma) := \frac 1 2 \pi(\vec\gamma)^\top \overline{\vec\Sigma}
\pi(\vec\gamma)
- \inner{\pi(\vec\gamma),\overline{\mv c}} + \frac\lambda 2 \Omega(\vec\gamma),$
where 
\begin{multline}
   \Omega(\vec\gamma) := 
   \sum_{w\notin F}\norm{\vec\gamma_w}^2
+ \sum_{i=1}^k \inner{(\vec\gamma_{f_i} - \vec\beta_{f_i}), \mv B_i^{-1}
   (\vec\gamma_{f_i} - \vec\beta_{f_i})}\\
+ \sum_{\ell=1}^r \sum_{w \notin \{f_1,\dots,f_k\}} \norm{\vec\gamma^{(\ell)}_w}^2
+ \sum_{\ell=1}^r \sum_{i=1}^k \norm{\vec\gamma^{(\ell)}_{f_i} - \sum_{c\in
   S_i}\mv R^\top_c \vec\gamma^{(\ell)}_c}^2,
   \label{eqn:omega:fama2}
\end{multline}
and $\pi(\vec\gamma)$ denotes the vector obtained from $\vec\gamma$ by removing
all components associated with $S_i,i\in [k]$.
\label{thm:fd:fama2}
\ethm

\noindent {\bf Remarks} 
As in the previous cases, we can say more. Suppose that the minimizer $\vec\gamma$ of $\overline J$
has been obtained, then a minimizer $\vec\theta$ of $J$ is available in closed form:
\begin{eqnarray*}
   \vec\theta_w &=& 
   \begin{cases}
      \vec\gamma_w & w \in V\setminus F\\
      \mv R_{t} \mv B_i^{-1} (\vec\gamma_{f_i} - \vec\beta_{f_i}), & \forall t \in F_i, i \in [k].
   \end{cases}\\
   \vec\theta_{w}^{(\ell)} &=& \vec\gamma_w^{(\ell)}, \qquad \forall w, \ell.
\end{eqnarray*}

In order to optimize $\overline J$ with respect to $\vec\gamma$,
the following proposition provides a closed form formulae for the relevant
gradient.
%; as is the case in $\pr$, the formulas reuse the
%computation of some components's gradients to compute other components's
%gradients, reducing computation time.

\bprop
The gradient of $\Omega(\vec\gamma)$ defined in~\eqref{eqn:omega:fama2} can
be computed by computing
$\vec\delta^{(\ell)}_{i} = \sum_{c\in S_i}\mv R_c^\top
\vec\gamma^{(\ell)}_c$, and
  \[ \vec\beta_{f_i} = \sum_{\ell=1}^r \left[ 
   \left(\vec\gamma^{(\ell)}_{f_i} - \frac 1 2 \vec\delta^{(\ell)}_{i} \right)\circ \vec\delta^{(\ell)}_{i}
   - \frac 1 2 \sum_{t \in S_i} \mv R^\top_t (\vec\gamma^{(\ell)}_t \circ \vec\gamma^{(\ell)}_t)
  \right]
  \]
Then,
\begin{align}
   \frac 1 2 \pd{\norm{\vec\theta}^2}{\vec\gamma_w} &=
   \begin{cases}
      \vec\gamma_w, & w \notin F\\
      \mv B_i^{-1}(\vec\gamma_{f_i}-\vec\beta_{f_i}) & w = f_i, i \in [k].
   \end{cases}\\
   \frac 1 2 \pd{\norm{\vec\theta}_2^2}{\vec\gamma^{(k)}_w}&=
   \begin{cases}
      \vec\gamma^{(k)}_w & w \notin F\\
      \displaystyle{
         \vec\gamma^{(k)}_{f_i} - \vec\delta^{(k)}_{i} \circ \left( \mv 1 + \frac 1 2 \pd{\norm{\vec\theta}_2^2}{\vec\gamma_{f_i}} \right)
}
      & w={f_i}\\
      \vec\gamma^{(k)}_w 
      - \mv R_w \left[ \vec\gamma_{f_i}^{(k)} \circ \frac 1 2 \pd{\norm{\vec\theta}_2^2}{\vec\gamma_{f_i}}
                  + \frac 1 2 \pd{\norm{\vec\theta}_2^2}{\vec\gamma_{f_i}^{(k)}}\right]
      & w \in S_i.
   \end{cases}
   \label{eqn:second:degree:fm:pd}
\end{align}
\label{prop:omega:fama2:gradient}
\eprop

